Implicit Multi-Spectral Transformer: An Lightweight and Effective Visible to Infrared Image Translation Model

In the field of computer vision, visible light images often exhibit low contrast in low-light conditions, presenting a significant challenge. While infrared imagery provides a potential solution, its utilization entails high costs and practical limitations. Recent advancements in deep learning, particularly the deployment of Generative Adversarial Networks (GANs), have facilitated the transformation of visible light images to infrared images. However, these methods often experience unstable training phases and may produce suboptimal outputs. To address these issues, we propose a novel end-to-end Transformer-based model that efficiently converts visible light images into high-fidelity infrared images. Initially, the Texture Mapping Module and Color Perception Adapter collaborate to extract texture and color features from the visible light image. The Dynamic Fusion Aggregation Module subsequently integrates these features. Finally, the transformation into an infrared image is refined through the synergistic action of the Color Perception Adapter and the Enhanced Perception Attention mechanism. Comprehensive benchmarking experiments confirm that our model outperforms existing methods, producing infrared images of markedly superior quality, both qualitatively and quantitatively. Furthermore, the proposed model enables more effective downstream applications for infrared images than other methods.

==> figtex/ab.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[b]{1.0\linewidth}
    \begin{minipage}[b]{0.49\linewidth}
        \centering
        \centerline{\includegraphics[width=\linewidth]{figs/ir_ab.jpg}}
        \centerline{(a) Target}\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\linewidth}
        \centering
        \centerline{\includegraphics[width=\linewidth]{figs/noagg.jpg}}
        \centerline{(b) Ours w/o DFA}\medskip
    \end{minipage}
    \end{minipage}
  \begin{minipage}[b]{1.0\linewidth}
    \begin{minipage}[b]{0.49\linewidth}
        \centering
        \centerline{\includegraphics[width=\linewidth]{figs/noatt.jpg}}
        \centerline{(c) Ours w/o EPA}\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\linewidth}
        \centering
        \centerline{\includegraphics[width=\linewidth]{figs/our.jpg}}
        \centerline{(d) Ours}\medskip
    \end{minipage}
  \end{minipage}
  \caption{
  Visual result of ablation study. (a) target infrared image. (b) our model without DFA. (c) our model without EPA. (d) our full model.
  } 
\label{fig:ab}
\end{figure}
